On construction schemes: building the uncountable from finite pieces

In this Phd. thesis, a structural analysis of construction schemes is developed. The importance of this study will be justified by constructing several distinct combinatorial objects which have been of great interest in mathematics. We then continue the study of capturing axioms associated to construction schemes. From them, we construct several uncountable structures whose existence is known to be independent from the usual axioms of Set Theory.

==> chapters/gaps.tex <==




\chapter{Gaps}
Consider the following situation: We have two Boolean algebras $\mathbb{A}\subseteq \mathbb{C}$ and an homomorphism $\phi$ from $\mathbb{A}$ to another Boolean algebra, say $\mathbb{B}$. For $x\in \mathbb{C}$, it is not necessarily the case that there is an 
homomorphism $\overline{\phi}:\mathbb{A}(x)\longrightarrow \mathbb{B}$ extending $\phi$. 
Let us define $L^\mathbb{A}_x$ as $\{y\in A\,:\,y\leq x\}$ and $U^A_x$ as $\{y\in 
\mathbb{A}\,\:\,y\geq x\}$. Whenever such $\overline{\phi}$ exists we can assure that 
there is an element of $\mathbb{B}$, namely $\overline{\phi}(x)$, for which $$\phi[L^\mathbb{A}_x]=\overline{\phi}[L^\mathbb{A}_x]\leq \overline{\phi}(x)\leq \overline{\phi}[U^\mathbb{A}_x]=\phi[U^\mathbb{A}_x].$$ 
This is just because $\overline{\phi}$ is order preserving. In \cite{Sikorskiextension}, Roman Sikorski implicitly proved that the converse also holds.
\begin{theorem}[Sikorski's extension criterion]\label{Sikorskitheorem}Let $\mathbb{A}$, $\mathbb{B}$ and $\mathbb{C}$ be Boolean algebras with $\mathbb{A}\subseteq \mathbb{C}$. Also let $x\in \mathbb{B}$ and $\phi:\mathbb{A}\longrightarrow \mathbb{B}$ be an homomorphism. If there is an element $y\in \mathbb{B}$ for which $\phi[L^\mathbb{A}_x]\leq y\leq \phi[U^\mathbb{A}_x]$ then there is an homomorphism $\overline{\phi}:\mathbb{A}(x)\longrightarrow \mathbb{B}$ extending $\phi$.
\begin{proof}Let $y$ be as in the hypotheses. As $\mathbb{A}(x)=\{a\cdot x+b\cdot(-x)\,:\,a,b \in \mathbb{A}\}$ we can define $\overline{\phi}:\mathbb{A}(x)\longrightarrow \mathbb{B}$ by:$$\overline{\phi}(a\cdot x+b\cdot(-x))=\phi(a)\cdot y+\phi(b)\cdot(-y).$$
Since each element of $\mathbb{A}(x)$ has many representations in the way described above, we still need to check that the definition of $\overline{\phi}$ does not depend on them.
\begin{claim}$\overline{\phi}$ is well defined.
\begin{proof}Let $a,a',b,b'\in \mathbb{A}$ be such that $a\cdot x+b\cdot(-x)=a'\cdot x+b'\cdot(-x).$ By multiplying by $x$ in both sides we get that $a\cdot x=a'\cdot x$. Observe that $(a+(-a'))\cdot x= x$ so $a+(-a')\in U^\mathbb{A}_x$. As $y\leq \phi[U^\mathbb{A}_x]$, we get $\phi(a)\cdot y+(-\phi(a'))\cdot y=\phi(a+(-a'))\cdot y= y$. Thus,
\begin{equation*}
\begin{split}
 \phi(a')\cdot y &= \phi(a')\cdot (\phi(a)\cdot y+(-\phi(a')\cdot y) \\  & = \phi(a)\cdot \phi(a')\cdot y \\   & \leq  \phi(a)\cdot y.
 \end{split}
\end{equation*}
Using that $((-a)+a')\cdot x=x$ we can deduce the other inequality, namely $\phi(a)\cdot y\leq \phi(a')\cdot y$. Furthermore, by coping the exact same argument but with $b$, $b'$ and $-x$ we get that $\phi(b)\cdot(-y)=\phi(b')\cdot(-y)$. Consequently $\phi(a)\cdot y+\phi(b)\cdot (-y)=\phi(a')\cdot y+\phi(b')\cdot (-y)$ which finishes the proof of the claim.
\end{proof}
\end{claim}
The only thing left to prove is that $\overline{\phi}$ is an homomorphism extending $\phi$. Such task is left to the reader.
\end{proof}

\end{theorem}

Independently of the existence of the extending homomorphism we always have that $\phi[L^\mathbb{A}_x]\leq \phi[U^\mathbb{A}_x]$.  Furthermore, $\phi[L^\mathbb{A}_x]$ is upwards directed and $\phi[U^\mathbb{A}_x]$ is downards directed. Thus, if we want to study in general the homorphisms ending in $\mathbb{B}$ and their possible extensions it is natural to study the pairs of subsets of $\mathbb{B}$ satisfying these conditions.  

\begin{definition}[Pre-gaps and Gaps]Let $\mathbb{B}$ be a boolean algebra and let $\mathcal{L}, \mathcal{U}$ be non-empty subsets of $\mathbb{B}$. We say that $(\mathcal{L},\mathcal{U})$ is a pre-gap if:
\begin{enumerate}[label=($\alph*$)]
\item $\mathcal{L}\leq \mathcal{U},$
\item $\mathcal{L}$ is upwards directed and $\mathcal{U}$ is downwards directed.
\end{enumerate}
A pre-gap $(\mathcal{L},\mathcal{U})$ is said to be filled by $x\in \mathbb{B}$ if $\mathcal{L}\leq x\leq \mathcal{U}$. In the case where no such $x$ exists we say that $(\mathcal{L},\mathcal{U})$ is a gap.
\end{definition}
Suppose that $(\mathcal{L},\mathcal{U})$ and $(\mathcal{L'},\mathcal{U}')$ are two pre-gaps in $\mathbb{B}$ such that $\mathcal{L}'$ is a cofinal subset of $\mathcal{L}$ and $\mathcal{U}'$ is a coinitial subset of $\mathcal{U}$.
Then it easy to see that $(\mathcal{L}',\mathcal{U}')$ is a gap if and only if the same is true for $(\mathcal{L},\mathcal{U})$. 
An important example of this situation arises when we consider a countable pre-gap $(\mathcal{L},\mathcal{U})$, that is,  with both $\mathcal{L}$ and $\mathcal{U}$ countable. Observe that in this case there is an increasing sequence  $\langle L_k\rangle_{k\in\omega}\subseteq \mathcal{L}$ cofinal in $\mathcal{L}$ and a decreasing sequence $\langle U_k\rangle_{k\in\omega}\subseteq \mathcal{U}$ coinitial in $\mathcal{U}$ respectively. In general it is easier to study the pre-gap determined by such sequences rather than the original one.

\begin{proposition}\label{nocountablegaps}$\mathscr{P}(\omega)/Fin$ has no countable gaps. 
\begin{proof}Let $(\mathcal{L},\mathcal{U})$ be a countable pre-gap in $\mathscr{P}(\omega)/Fin$. Due to the observation preceeding this proposition, we can assume that $\mathcal{L}$ is of the form $\langle[L_k]\rangle_{k\in\omega}$ for a $\subseteq^*$-increasing sequence in $\mathscr{P}(\omega)$ and $\mathcal{U}$ is of the form $\langle [U_k]\rangle_{k\in\omega} $ for a $\subseteq^*$-decreasing sequence in $\mathscr{P}(\omega)$. Define $X$ as $$\bigcup\limits_{k\in\omega}\big(L_k\cap(\bigcap\limits_{i\leq k}U_k)\big).$$ Since $L_k\subseteq^* L_k\cap (\bigcap\limits_{i\leq k}U_i)$ for each $k\in\omega$ it follows that $\mathcal{L}\leq [X]$. On the other hand, since $L_j\cap(\bigcap_{i\leq j}U_i)\subseteq U_k$ for each $k\in\omega$ and every $j\geq k$ we have that $[X]\leq \mathcal{U}.$ We conclude that $(\mathcal{L},\mathcal{U})$ is filled by $[X]$.\end{proof}
\end{proposition}
\begin{corollary}\label{homomorphismextension}Let $\mathbb{A}$ and $\mathbb{B}$ be two boolean algebras such that $|\mathbb{A}|\leq \omega$ and $|\mathbb{B}|\leq \omega_1$. Every homomorphism from $\mathbb{A}$ to $\mathscr{P}(\omega)/Fin$ can be extended to $\mathbb{B}$.
\begin{proof}Let $\phi:\mathbb{A}\longrightarrow \mathscr{P}(\omega)/Fin$ be a homomorphism. As $\mathbb{B}$ has cardinality at most $\omega_1$ we can enumerate it (possibly with repetitions) as $\langle b_\alpha \rangle_{\alpha\in \omega_1}$. 
For each $\alpha\in \omega_1$ define $\mathbb{A}_\alpha$ as $\langle \mathbb{A}\cup \{b_\xi\,:\,\xi<\alpha\}\rangle$. Observe that $\mathbb{A}_0=\mathbb{A}$. Furthermore, if $\beta=\alpha+1$ then $\mathbb{A}_\beta=\mathbb{A}_\alpha(b_\alpha)$ and if $\gamma$ is 
limit then $\mathbb{A}_\gamma=\bigcup\limits_{\alpha<\gamma}\mathbb{A}_\alpha$. We now define recursively a sequence $\langle \phi_\alpha\rangle_{\alpha\in\omega_1}$ of homomorphisms such that:
\begin{enumerate}
\item $\phi_0=\phi$.
\item $\phi_\alpha:\mathbb{A}_\alpha\longrightarrow \mathscr{P}(\omega)/Fin$ for each $\alpha\in\omega_1$.
\item $\phi_\beta$ extends $\phi_\alpha$ whenever $\alpha<\beta$.
\end{enumerate}
 For the construction we consider the limit and succesor case. If $\gamma$ is a limit ordinal and we have defined $\phi_\alpha$ for each $\alpha<\gamma$, we simply define $\phi_\gamma$ as the union of the previous $\phi_\alpha$'s. For the succesor step, suppose that $\alpha\in\omega_1$ and we have define $\phi_\alpha$. Note that since $\mathbb{A}_\alpha$ is countable then $(\phi_\alpha[L^{\mathbb{A}_\alpha}_\alpha],\phi_\alpha[U^{\mathbb{A}_\alpha}_{\alpha}])$ is a countable pre-gap in $\mathscr{P}(\omega)/Fin$. Due to Proposition \ref{nocountablegaps} such a pre-gap can be filled so by \textit{Sikorski's extension criterion} there is an homomorphism $\phi_{\alpha+1}:\mathbb{A}_{\alpha+1}\longrightarrow \mathscr{P}(\omega)/Fin$ extending $\phi_\alpha$.\\
 To finish the proof let $\phi:\mathbb{B}\longrightarrow \mathscr{P}(\omega)/Fin$ be defined as $\bigcup\limits_{\alpha\in\omega_1}\phi_\alpha$. It is straightforward that such $\phi$ does the job.
\end{proof}
\end{corollary}
\begin{definition}[Pre-towers and Towers]Let $\mathbb{B}$ be a boolean algebra. We call pre-towers to all non-empty well ordered subsets of $\mathbb{B}\backslash \{\mathbbm{1}\}.$ A pre-tower $\mathcal{T}$ in $\mathbb{B}$ is said to be a tower if there is no $x\in \mathcal{B}\backslash \{\mathbbm{1}\}$ with $\mathcal{T}<x$. Additionally we say that $\mathcal{T}'\subseteq \mathbb{B}^+$ is a decreasing pre-tower if $-\mathcal{T}':=\{-t\,:\,t\in \mathcal{T}\}$ is a pre-tower, and we say that $\mathcal{T}'$ is a decreasing tower if $-\mathcal{T}'$ is a tower.
\end{definition}
As well as in the case of gaps it is easy to see that if $\mathcal{T}$ is a pre-tower and $\mathcal{T}'$ is a cofinal subset of $\mathcal{T}$ then $\mathcal{T}'$ is a tower if and only if the same holds for $\mathcal{T}$. An analogous statement is true when we talk about descreasing pre-towers and we change \say{cofinal} by \say{coinitial}. By these observations it is easy to see that the atomless algebras are exactly those which have no towers with maximal elements.
The following result is well knownn
\begin{proposition}$\mathscr{P}(\omega)/Fin$ has no countable towers.
\begin{proof}Let $\mathcal{T}$ be a countable pre-tower. Since $\mathscr{P}(\omega)/Fin$ is atomless we can assume without loss of generality that $\mathcal{T}$ has no maximal element. Hence, there is a strictly increasing sequence $\langle [T_k]\rangle_{k\in\omega}\subseteq \mathcal{T}$ cofinal in $\mathcal{T}$. By the observation preceding this proposition, it is enough to show that such sequence is not a tower. For this, recursively pick for each $k\in\omega$ an $x_k\in \omega\backslash (\bigcup\limits_{i\leq {k+1}} T_i)$ in such way that $x_k\not=x_j$ whenever $k\not=j$. Now define $X$ as $\{x_k\,:\,k\in\omega\}$ . We claim that $[\omega \backslash X]$ testifies what we want to prove. First observe that since $X$ is infinite, $[\omega\backslash X]<[\omega]$. Also note that $T_k\backslash(\omega\backslash X)\subseteq \{x_i\,:i< k\}$ for each $k$. As the sequence is strictly increasing,  $\langle [T_k]\rangle_{k\in\omega}<[\omega\backslash X]$. So we are done. 
\end{proof}
\end{proposition}
\begin{definition}Let $\mathbb{B}$ be a boolean algebra, $x\in \mathbb{B}$ and $(\mathcal{L},\mathcal{U})$ be a pre-gap in $\mathbb{B}$. We say that $(\mathcal{L},\mathcal{U})$ is strongly filled by $x$ if $\mathcal{L}<x<\mathcal{U}$.
\end{definition}
\begin{lemma}Let $\mathbb{B}$ be a boolean algebra with neither countable gaps nor countable towers. Then every countable pre-gap in $\mathbb{B}$ is strongly filled by some element.
\begin{proof}Let $(\mathcal{L},\mathcal{U})$ be a countable pre-gap in $\mathbb{B}$. It is safe to assume that $\mathcal{L}$ is a pre-tower and $\mathcal{U}$ is a decreasing pre-tower. As $\mathbb{B}$ has no countable gaps there is $x\in \mathbb{B}$ which fills $(\mathcal{L},\mathcal{U})$.

\begin{claim}There is $y\in \mathbb{B}$ such that  $\mathcal{L}<y\leq \mathcal{U}$.
\begin{proof}If $x\notin\mathcal{L}$ then $y=x$ works, so suppose that $x\in \mathcal{L}$. As $\mathcal{L}<\mathcal{U}$ this means that $x<\mathcal{U}$. Define $\mathcal{U}'$ as $\{a\cdot(-x)\,:\,x\in \mathcal{U}\}$. Then $\mathcal{U}'\subseteq \mathbb{B}^+$ is also a decreasing pre-tower in $\mathbb{B}$. Since $\mathbb{B}$ has no countable towers, there is $y'\in \mathbb{B}$ with $\mathbb{0}<y'<\mathbb{U}'$. To finish, define $y$ as $x+y'$. It is straightforward that $\mathcal{L}\leq x<y< \mathcal{U}$.
\end{proof}
\end{claim}
Let $y\in \mathbb{B}$ as in the previous claim. Define $\mathcal{L}'$ as $\{a+(-y)\,:\,a\in \mathcal{L}\}$.  Then $\mathcal{L}$ is a countable pre-tower in $\mathbb{B}$. As $\mathbb{B}$ has no countable pretowers, there is $z\in \mathbb{B}$ with $\mathcal{L}'<z<\mathbbm{1}$. It is easy to check that $\mathcal{L}<z\cdot y<y$. That is,  $(\mathcal{L},\mathcal{U})$  is strongly filled by $z\cdot y.$
\end{proof}
\end{lemma}

\begin{definition}A Boolean algebra $\mathbb{B}$ is called a Parovi\v{c}enko algebra if every countable pre-gap in $\mathbb{B}$ is strongly filled by some element.
\end{definition}


\begin{lemma}\label{parovicenkolemma}Let $\mathbb{B}$ be a Parovi\v{c}enko algebra and let $\mathcal{L}$, $\mathcal{U}$ and $Z$ be non-empty countable subsets of $\mathbb{B}$ with the following properties:
\begin{enumerate}
\item $(\mathcal{L},\mathcal{U})$ is a pre-gap,
\item $z\cdot(-a)>\mathbb{0}$ for each $a\in \mathcal{L}$ and $z\in Z,$
\item $z\cdot c>\mathbb{0}$ for each $c\in \mathcal{U}$ and $z\in Z$.
\end{enumerate}
Then there is $b\in \mathbb{B}$ strongly filling $(\mathcal{L},\mathcal{U})$ and such that $z\cdot (-b)>\mathbb{0}$ and $z\cdot b>\mathbb{0}$ for each $z\in Z.$
\end{lemma}

\begin{theorem}[Sikorski's extension criterion for embeddings]\label{Sikorskiextensionemb}Let $\mathbb{A},$ $\mathbb{B}$ and $\mathbb{C}$ be Boolean algebras with $\mathbb{A}\subseteq \mathbb{C}$. Also let $x\in \mathbb{B}$, $\phi:\mathbb{A}\longrightarrow \mathbb{B}$ be an embedding. If there is $y\in \mathbb{B}$ is such that:\begin{enumerate}[label=$(\arabic*)$]
\item the pre-gap $(\phi[L^\mathbb{A}_x],\phi[U^\mathbb{A}_x])$,
\item $\phi(a)\cdot y>0$ for each $a\in \mathbb{A}$ with $a\cdot x>\mathbb{0}$ and 
\item $\phi(a)\cdot (-y)>0$ for each $a\in \mathbb{A}$ with $a\cdot (-x)>\mathbb{0},$
\end{enumerate}
then there is an embedding $\overline{\phi}:\mathbb{A}(x)\longrightarrow \mathbb{B}$ extending $\phi.$
\end{theorem}
Equipped with Lemma \ref{parovicenkolemma} and \textit{Sikorski's extension criterion for embeddings}, one can modify the proof of Corollary \ref{homomorphismextension} by means of a transfinite back and forth argument in order to prove the following theorem due to I. I. Paravi\v{c}enko. This theorem was originally proved in \cite{parovicenko}. The reader interested in a complete proof can find it in \cite{gapsandlimits} and \cite{handbookbooleanalgebras}.

\begin{theorem}[Parovi\v{c}enko's Theorem] Any two Paravi\v{c}enko algebras of size $\omega_1$ are isomorphic. In particular, under $CH$ every Paravi\v{c}enko algebra is isomorphic to $\mathscr{P}(\omega)/Fin$.
\end{theorem}

\section{Uncountablegaps}
Part of the previous section was dedicated to study the non-existence of countable gaps in boolean algebras. As we saw earlier, the importance of this study radicates in its relation with the existence of extensions of both homomorphisms and embeddings. Although easy to prove, the non-existence of countable gaps in $\mathscr{P}(\omega)/Fin$ is such a deep result that it allow us to characterize this algebra under the Continuum Hypothesis. Unfortunately, when we take CH out of the equation the situation becomes more complicated. Gaps do exist in $\mathscr{P}(\omega)/Fin$. In fact, their existence can be easily deduced by a simple application of Zorn's Lemma. However, there is not to much to say about the structure of the gaps given by this method when used in a careless way. In this rest of this chapter, we will use schemes to construct various types of gaps in $\mathscr{P}(\omega)/Fin$ with strong combinatorial properties. But first we will make  based on the following remarks.
\begin{remark}Let $(\mathcal{L},\mathcal{U})$ be a pre-gap in a boolean algebra $\mathbb{B}$. Then the pair $(\mathcal{L},-\mathcal{U})$ satisfies the following properties:
\begin{itemize}
\item Both $\mathcal{L}$ and $-\mathcal{U}$ are upward directed,
\item $\mathcal{L}$ and $\mathcal{U}$ are orthogonal, that is, $a\cdot b=\mathbb{0}$ for each $a\in\mathcal{L}$ and $b\in-\mathcal{U}$.
\end{itemize}
Note that if $\mathcal{L}'$ and $\mathcal{U}'$ are two orthogonal non-empty upwards directed subsets of $\mathbb{B}$ then $(\mathcal{L}',-\mathcal{U}')$ is a pre-gap. Thus, study of such pairs is equivalent to the study of pre-gaps. 
\end{remark}
\begin{remark}Any pre-gap $(\mathcal{L},\mathcal{U})$ in $\mathscr{P}(\omega)/Fin$ is determined by two families of subsets of $\omega$, say $L$ and $U$, with the following properties:
\begin{itemize}
\item $L$ is upwards directed with respect to $\subseteq^*$,
\item $U$ is downwards directed with respect to $\subseteq^*$,
\item $A\subseteq^*B$ for all $A\in L$ and $B\in U$.
\end{itemize}
\end{remark}
Based on the previous remarks we now define gaps and towers in $\mathscr{P}(\omega)$.
\begin{definition}[towers in $\mathscr{P}(\omega)$]Let $\mathcal{T}$ be a non-empty subset of $\mathscr{P}(\omega)$. We say that $\mathcal{T}$ is a pretower if it is well ordered with respect to $\subseteq^*.$  Additionally, if $ot(\mathcal{T})=\kappa$ we may call $\mathcal{T}$ a $\kappa$-pretower.
\end{definition}
Whenever we index a pretower with an ordered set it is understood that this is done in an order increasing way.
\begin{definition}[$(\kappa,\lambda)$-gaps in $\mathscr{P}(\omega)$]Let $\mathcal{A},\mathcal{B}$ be non-empty subsets of $\mathscr{P}(\omega)$ and $\kappa,\lambda$ be arbitrary cardinals. We say that $(\mathcal{A},\mathcal{B})$ is a $(\kappa,\lambda)$-pregap if:
\begin{enumerate}[label=$(\alph*)$]
\item $\mathcal{A}$ is a $\kappa$-pretower,
\item $\mathcal{B}$ is a $\lambda$-pretower,
\item $A\cap B=^*\emptyset$ for al $A\in \mathcal{A}$ and $B\in \mathcal{B}.$
\end{enumerate}
Additionally, if there is no $C\in [\omega]^{\omega}$ with $A\subseteq^*C$ and $B\cap C=^*\emptyset$ for  all $A\in \mathcal{A}$ and $B\in \mathcal{B}$ then we say that $(\mathcal{A},\mathcal{B})$ is a pregap. Whenever such $C$ exists we say that $C$ separates $(\mathcal{A},\mathcal{B}).$
\end{definition}
In 1909, Felix Hausdorff gave a clever construction of an $(\omega_1,\omega_1)$-gap without appealing to any extra axioms.
Due to some descriptive set theoretic aspects, most \say{nice} definable objects (related to $\omega$) which can be constructed from $ZFC$ are either countable or of size $\mathfrak{c}$. This may be one of the many reasons why, even to this day, Hausdorff's construction is still impressive and its proof technique is deeply rooted in the minds of a great part of the set theoretic community.\\
A natural way of constructing an $(\omega_1,\omega_1)$-gap is through the use of a transfinite recursion of length $\omega_1$. At each step $\beta$ we find $A_\beta,B_\beta\in [\omega_1]^{\omega}$ satisfying the expected properties:
\begin{enumerate}[label=$(\arabic*)$]
\item $A_\alpha\cap B_\alpha=^*\emptyset$,
\item $A_\alpha\subsetneq^*A_\beta$ and $B_\alpha\subsetneq^*B_\beta$ for each $\alpha<\beta.$
\end{enumerate}
 If we are not careful enough it may be impossible to find $A_\alpha$ and $B_\alpha$ satisfying property $(2)$. This is easily fixed if we also ask for the following recursion hypothesis to hold:
\begin{center}
($RI_1$)$\:$For each $\alpha\in \omega_1$, $\omega\backslash (A_\alpha\cup B_\alpha)$ is infinite.
\end{center}
Of course, the resulting construction will produce an $(\omega_1,\omega_1)$-pre-gap consisting of the sequences $\mathcal{A}:=\langle A_\alpha\rangle_{\alpha\in \omega_1}$ and $\mathcal{B}:=\langle B_\alpha\rangle_{\alpha\in \omega_1}$. However, there is no reason to expect such a pregap to be a gap. Here is where the real problem arises; Given $C\in [\omega]$ and $\beta\in \omega_1$ it is possible to construct $A_\beta$ and $B_\beta$ in such way that $C$ does not separate $(\langle A_\alpha\rangle_{\alpha\leq \beta},\langle B_\alpha\rangle_{\alpha\leq \beta})$. Note that in this case $C$ won't separate $(\mathcal{A},\mathcal{B})$ neither. Hence, if we assume $CH$ and we index $[\omega]^{\omega}$ as $\langle C_\alpha\rangle_{\alpha\in \omega_1}$ then the following recursion hypothesis will prophesy the \say{gapness} of $(\mathcal{A},\mathcal{B})$:
\begin{center}($RI_{CH}$)$\:$ For each $\beta\in \omega_1$, $C_\beta$ does not separate 
$(\langle A_\alpha\rangle_{\alpha\leq \beta},\langle B_\alpha\rangle_{\alpha\leq \beta})$.
\end{center}
The problem with the core of the previous argument and the negation of $CH$ can be resumed in the frase \say{too many tasks and too little time}. 

==> chapters/nosuslin.tex <==
\chapter{No Suslin trees from $\mathfrak{m}_\mathcal{F}>\omega_1$}
For the rest of this section, we fix a $\clubsuit$-sequence $\langle C_\gamma\rangle_{\gamma\in \text{Lim}}$ and construction scheme $\mathcal{F}$ over a limit ordinal $\gamma$.

\begin{definition}Let us denote $\text{Lim}$ as $\mathcal{L}_0$.  Given $0<n\in\omega$, we recursively define $$\mathcal{L}_n=\{\gamma\in \text{Lim}\,:\,\forall \alpha\in C_\gamma\,(\,C_\alpha\subseteq \mathcal{L}_{n-1}\,)\}.$$
\end{definition}
\begin{definition}
Let $C^0_\gamma=C_\gamma$ for each $\gamma\in \mathcal{L}_0$. Given $0<n\in\omega$ and $\gamma\in \mathcal{L}_n$, we recursively define $$C^n_\gamma=\bigcup\limits_{\alpha\in C_\gamma} C^{n-1}_\alpha.$$
\end{definition}

\begin{proposition}Let $X\in [\omega_1]^{\omega_1}$. Given $n\in\omega$, there is $\gamma\in \mathcal{L}_n$ such that $C^n_\gamma\subseteq X.$ 
\end{proposition}
\begin{definition}[$IH^\clubsuit_n$]Let $n\in\omega$ and $\beta\in \mathcal{L}_n$  be such that $\beta\leq \gamma$. Suppose that $A\in \text{FIN}(\gamma)$ is such that $A\cap \beta\not=\emptyset$. Given $F\in \mathcal{F}$, we say that $IH^\clubsuit_{\beta,n}(A,F)$ holds if:
\begin{itemize}
\item $n_{\rho^F}>n.$
    \item $A\subseteq F_n$ and $\max(A\cap \alpha)=\max(R(F))$.
    \item There is $D\in [C^n_\beta]^{n}$ so that $D(i)\in F_i\backslash R(F)$ for each $i<n$.
\end{itemize}
Additionally, $\mathcal{F}$ is said to satisfy $IH^\clubsuit_{\beta,n}$ if for each $A\in \text{FIN}(\gamma)$ as above, there is $F\in\mathcal{F}$ for which $IH^\clubsuit_{\beta,n}(A,F)$ holds.
\end{definition}
\begin{lemma}Let $\beta\in \mathcal{L}_0$ be such that $\beta\leq \gamma$. If $\mathcal{F}$ satisfies $IH_1$, then it also satisfies $IH^\clubsuit_{\beta,0}.$   
\end{lemma}
\begin{lemma}Let $0<n\in\omega$ and suppose that $\gamma\in \mathcal{L}_n$. If $\mathcal{F}$ satisfies $IH^\clubsuit_{\beta,n-1}$ for each $\beta\in C^n_\gamma$, then $\mathbb{P}(\mathcal{F})\Vdash$
    
\end{lemma}
    








 

==> chapters/proyection.tex <==
 As the $k$-closures of $A$ and $B$ have size at most $m_k$, it is natural to code the type such arrangements as subsets of $m_k$. The following definition formalizes this idea.


\begin{definition}[The projection] Let $A\in \text{FIN}(X)$ and $k\geq \rho^A$. We define the \textit{$k$-projection}, of $A$ as $$\pi_k A=(A)_{k}^{-1}[A]\subseteq m_k.$$
 In the case where $k=\rho^A$, we denote $\pi_kA$ simply as $\pi A$ and call it the \textit{projection} of $A$. 
\end{definition}


\begin{rem}If we take $i\leq \lVert \max(A)\rVert$ then $i\in \pi_k A$ if and only if $(A)_k(i)\in A$. Furthermore,  $(A)_k[\pi_k A]=A$ and $\max(\pi_k A)=\lVert\max(A)\rVert_k$. In particular, this means that for given $A$ and $B$ in $FIN(X)$,  $\pi_k A=\pi_k B$ if and only if $(A)_k$ is $\rho$-isomorphic to $(B)_k$ and the increasing bijection between these two sets sends $A$ to $B$.
\end{rem}
In the following two lemmas we analyze sufficient conditions under which $\pi_k A$ equals $\pi_k B$. 
\begin{lemma}\label{lemmaproyectiondown}Let $A,B\in \text{FIN}(X)$ and $l\geq \max(\rho^A,\rho^B)$. If $\pi_l A=\pi_l B$ then $\rho^A=\rho^B$ and $\pi_k A=\pi_k B$ for each $k\in\omega$ with $\rho^A\leq k\leq l$.

\begin{proof} First we prove that $\rho^A=\rho^B$. Let $S=\pi_l A$. By the previous remark we have that $\lVert\max(A)\rVert_l=\lVert \max(B)\rVert_l$.  In this way $(\max(A))_l=(A)_l$ and $(\max(B))_l=(B)_l$ are $\rho$-isomorphic due to Corollary \ref{ballhomogeneitylemma}. Since $(A)_l[S]=A$ and $(B)_l[S]=B$ then
\begin{align*}\rho^A &=\max(\, \rho((A)_l(i),(A)_l(j))\,:\,i,j\in S\,)\\
&=\max(\, \rho((B)_l(i),(B)_l(j))\,:\,i,j\in S\,)
=\rho^B.
\end{align*}
Now we prove that $\pi_k A\subseteq \pi_k B$ for any $k$ as in the hypotheses. For this  consider $h:(A)_l\longrightarrow (B)_l$ to be the increasing bijection. By the previous remark, as $\pi_l A=\pi_l B$ then $h[A]=B$. Since $\rho^A=\rho^B\leq k\leq l$ then $(A)_k\subseteq (A)_l$ and $(A)_k=(\max(A))_k$. Analogously with $B$. Furthermore, as $h(\max(A))=\max(B)$ we conclude that $$h[(A)_k]=h[(\max(A))_k]=(\max (B))_k=(B)_k.$$
This means that $h|_{(A)_k}$ is the (only) increasing bijection between $(A)_k$ and $(B)_k$. Therefore $h[(A)_k(j)]=(B)_k(j)$ for any $j\leq |(A)_k|$. Now let $i\in \pi_k A$. Then $(A)_k(i)\in A$ so by the previous observation $(B)_k(i)=h[(A)_k(i)]\in B$. Consequently $i\in \pi_k B$. This proves that $\pi_k A\subseteq \pi_k B$. The proof of $\pi_k B\subseteq \pi_k A$ is completely analogous.

\end{proof}
\end{lemma}
\begin{lemma}Let $A,B\in \text{FIN}(X)$ with $\rho^A=\rho^B$. If $\pi A=\pi B$ and $k\in\omega$ is such that $k\geq \rho^A$ and $\lVert \max(A)\rVert_k=\lVert \max(B)\rVert_k$ then $\pi_k A=\pi_k B$
\begin{proof}By Corollary \ref{ballhomogeneitylemma} we have that $(\max(A))_k=(A)_k$ is $\rho$-isomorphic to $(\max(B))_k=(B)_k$. Let $h:(A)_k\longrightarrow (B)_k$ be the (only) increasing bijection. Note that $$h[(A)_{\rho^A}]=h[(\max(A))_{\rho^A}]=(\max(B))_{\rho^A}=(B)_{\rho^B}.$$
As in the third paragraph of the proof of Lemma \ref{lemmaproyectiondown}, this implies that $h[(A)_{\rho^A}(j)]=(B)_{\rho^B}(j)$ for each $j\leq |(A)_k|$. Let $i\in \pi_k A$. Then $(A)_k(i)\in A= (A)_{\rho^A}[\pi A]$. Hence, there is $j\in \rho^A$ such that $(A)_{\rho^A}(j)=(A)_k(i)$. It follows that
$$(B)_k(i)=h[(A)_k(i)]=h[(A)_{\rho^A}(j)]=(B)_{\rho^B}(j).$$
Since $\pi A=\pi B$ then $j\in \pi B$. Therefore $(B)_k(i)\in B$ which means that $i\in \pi_k B$. This proves that $\pi_k A\subseteq \pi_k B$. The other contention is proved in an analogous way.
\end{proof}
\end{lemma}
